Revisit the Partial Coloring Method: Prefix Spencer and Sampling

As the most powerful tool in discrepancy theory, the partial coloring method has wide applications in many problems including the Beck-Fiala problem and Spencer's celebrated result. Currently, there are two major algorithmic methods for the partial coloring method: the first approach uses linear algebraic tools; and the second is called Gaussian measure algorithm. We explore the advantages of these two methods and show the following results for them separately. 1. Spencer conjectured that the prefix discrepancy of any $\mathbf{A} \in \{0,1\}^{m \times n}$ is $O(\sqrt{m})$. We show how to find a partial coloring with prefix discrepancy $O(\sqrt{m})$ and $\Omega(n)$ entries in $\{ \pm 1\}$ efficiently. To the best of our knowledge, this provides the first partial coloring whose prefix discrepancy is almost optimal. However, unlike the classical discrepancy problem, there is no reduction on the number of variables $n$ for the prefix problem. By recursively applying partial coloring, we obtain a full coloring with prefix discrepancy $O(\sqrt{m} \cdot \log \frac{O(n)}{m})$. Prior to this work, the best bounds of the prefix Spencer conjecture for arbitrarily large $n$ were $2m$ and $O(\sqrt{m \log n})$. 2. Our second result extends the first linear algebraic approach to a sampling algorithm in Spencer's classical setting. On the first hand, Spencer proved that there are $1.99^m$ good colorings with discrepancy $O(\sqrt{m})$. Hence a natural question is to design efficient random sampling algorithms in Spencer's setting. On the other hand, some applications of discrepancy theory, prefer a random solution instead of a fixed one. Our second result is an efficient sampling algorithm whose random output has min-entropy $\Omega(n)$ and discrepancy $O(\sqrt{m})$. Moreover, our technique extends the linear algebraic framework by incorporating leverage scores of randomized matrix algorithms.

==> subGaussian_RW.tex <==
\subsection{Full coloring algorithm under Banaszczyk's setting}

\subsubsection{1-dimension case}
We will continue using the notations defined earlier in this discussion. In the one-dimensional setting, we propose an alternative random walk as follows:
\begin{definition}[1-dimension random walk]
Given $\omega_n$ and $v_{n+1}$, the $(n+1)$-th location is $x_{n+1}=\frac{\langle \omega_{n},v_{n+1}\rangle}{|v_{n+1}|} = \omega_{n}\cdot \operatorname{sgn}(v_{n+1})$. The next assignment, $\epsilon_{n+1}$, is defined as:
\begin{equation}
\label{eq6}
\epsilon_{n+1}=\left\{
\begin{aligned}
1 &  \textit{ with prob. } q(x_{n+1},|v_{n+1}|), \textit{ for } x_{n+1} \ge |v_{n+1}| \\
-1 &  \textit{ with prob. } 1-q(x_{n+1},|v_{n+1}|), \textit{ for } x_{n+1} \ge |v_{n+1}| \\
1 &  \textit{ with prob. } 0.5, \textit{ for } |v_{n+1}| \ge  x_{n+1} \ge -|v_{n+1}| \\
-1 &  \textit{ with prob. } 0.5, \textit{ for } |v_{n+1}| \ge  x_{n+1} \ge -|v_{n+1}| \\
1 &  \textit{ with prob. } 1-q(-x_{n+1},|v_{n+1}|), \textit{ for } x_{n+1} \le -|v_{n+1}| \\
-1 &  \textit{ with prob. } q(-x_{n+1},|v_{n+1}|), \textit{ for } x_{n+1} \le -|v_{n+1}| \\
\end{aligned}
\right.
\end{equation}
where the transition probability $q(x,y)=e^{-3xy}-e^{-4xy}$.
\end{definition}

\begin{claim}
For all $n\in \mathbb{N}$, $\omega_{n}$ is sub-gaussian.
\end{claim}
\begin{proof}
W.l.o.g let $\omega_{0}=1$ and $x_{n+1}\ge -|v_{n+1}|$. For $|v_{n+1}|> x_{n+1}\ge -|v_{n+1}|$, we have $|w_{n}|\le 1$, which means $|\omega_{n+1}|\le 2$. For $x_{n+1}\ge |v_{n+1}|$,  \begin{align}
    \E_{\epsilon_{n+1}}[e^{|\omega_{n+1}|^{2}}] &= \E_{\epsilon_{n+1}}[e^{\omega_{n}^{2}+|v_{n+1}|^{2}+2\cdot \epsilon_{n+1}\cdot \omega_{n}\cdot v_{n+1}}]\\
    &= \E_{\epsilon_{n+1}}[e^{\omega_{n}^{2}+|v_{n+1}|^{2}+2\cdot \epsilon_{n+1}\cdot x_{n+1}\cdot |v_{n+1}|}]\\
    &\le e^{\omega_{n}^{2}+|v_{n+1}|^{2}}\cdot \left(e^{-2\cdot x_{n+1}\cdot|v_{n+1}|}+q\left(x_{n+1},|v_{n+1}|\right)\cdot e^{2\cdot x_{n+1}\cdot |v_{n+1}|}\right)\\
    &= e^{\omega_{n}^{2}+|v_{n+1}|^{2}-x_{n+1}\cdot |v_{n+1}|}\\
    &\le e^{|\omega_{n}|^{2}}
\end{align}
so that $\E[e^{|\omega_{n+1}|^{2}}]\le \E[e^{|\omega_{n}|^{2}}]\le \E[e^{|\omega_{0}|^{2}}]=e$. In a word, 
we have $\E[e^{|\omega_{n}|^{2}}]\le e^{4}$ which means $\omega_{n}$ is sub-gaussian with parameter $\lambda =1$.
\end{proof}
More generally, for any direction $u\in \R^{n}$ with $\|u\|_{2}=1$, we prove $\langle\omega_{n},u\rangle$ is a sub-gaussian satisfying $\mathop{\E}\limits_{\omega_{n}}[e^{\langle\omega_{n},u\rangle^{2}}]\le e^{4}$ for any $n\in N$.

Given $v_{i+1}$ and $\omega_{i}$, suppose we have $\mathop{\E}\limits_{\omega_{n}}[e^{\langle\omega_{n},u\rangle^{2}}]\le e^{4}$. By definition we have \begin{align}
    \mathop{\E}\limits_{\omega_{i+1}}[e^{\langle\omega_{i+1},u\rangle^{2}}] &= \mathop{\E}\limits_{\omega_{i}} \{e^{\langle\omega_{i},u\rangle^{2}}\mathop{\E}\limits_{\epsilon_{i+1}}[exp(\langle v_{i+1},u\rangle^{2}+2\cdot\epsilon_{i+1}\langle \cdot \omega_{i},u\rangle \cdot \langle v_{i+1},u\rangle)]\}\\
    &=\mathop{\E}\limits_{\omega_{i}} \{e^{\langle\omega_{i},u\rangle^{2}+\langle v_{i+1},u\rangle^{2}}\mathop{\E}\limits_{\epsilon_{i+1}}[exp(2\cdot\epsilon_{i+1}\langle \cdot \omega_{i},u\rangle \cdot \langle v_{i+1},u\rangle)]\}, \label{eq_hy_in_subgaussian}
\end{align}

If $u\perp v_{i+1}$:  $\mathop{\E}\limits_{\omega_{i+1}}[e^{\langle\omega_{i+1},u\rangle^{2}}]=\mathop{\E}\limits_{\omega_{i}}[e^{\langle\omega_{i},u\rangle^{2}}]\le e^{4}$.

If $u$, $v_{i+1}$ are not orthogonal while $u\perp\omega_{i}$: $\mathop{\E}\limits_{\omega_{i+1}}[e^{\langle\omega_{i},u\rangle^{2}}]=1 $, so we have $\mathop{\E}\limits_{\omega_{i+1}}[e^{\langle \omega_{i+1},u\rangle^{2}}]=e^{\langle v_{i+1},u\rangle^{2}}\le e\le e^{4} $.

If $u$, $v_{i+1}$ and $u$, $\omega_{i}$ are both not orthogonal: let $x_{i+1}=\frac{\langle\omega_{i},u\rangle\cdot \langle v_{i+1},u\rangle}{\|v_{i+1}\|_{2}}$ and condiser the random walk defined in 1-dimensional case, namely \begin{equation}
\label{eq6}
\epsilon_{i+1}=\left\{
\begin{aligned}
1 &  \textit{ with prob. } q(x_{i+1},|v_{n+1}|), \textit{ for } x_{i+1} \ge \|v_{i+1}\|_{2} \\
-1 &  \textit{ with prob. } 1-q(x_{i+1},\|v_{i+1}\|_{2}), \textit{ for } x_{i+1} \ge \|v_{i+1}\|_{2} \\
1 &  \textit{ with prob. } 0.5, \textit{ for } \|v_{i+1}\|_{2} \ge  x_{i+1} \ge -\|v_{i+1}\|_{2} \\
-1 &  \textit{ with prob. } 0.5, \textit{ for } \|v_{i+1}\|_{2} \ge  x_{i+1} \ge -\|v_{i+1}\|_{2} \\
1 &  \textit{ with prob. } 1-q(-x_{i+1},\|v_{i+1}\|_{2}), \textit{ for } x_{i+1} \le -\|v_{i+1}\|_{2} \\
-1 &  \textit{ with prob. } q(-x_{i+1},\|v_{i+1}\|_{2}), \textit{ for } x_{i+1} \le -\|v_{i+1}\|_{2} \\
\end{aligned}
\right.
\end{equation}
where the transition probability $q(x,y)=e^{-3xy}-e^{-4xy}$. If $-\|v_{i+1}\|_{2}\le x_{i+21}\le \|v_{i+1}\|_{2}$, \begin{equation}
    |\langle\omega_{i},u\rangle\cdot \langle v_{i+1},u\rangle|\le \|v_{i+1}\|_{2}^{2}\le 1,
\end{equation}
which means $|\langle\omega_{i},u\rangle|\le 1$
so we have \begin{equation}
    |\langle \omega_{i+1},u\rangle|=|\langle \omega_{i},u\rangle+\epsilon_{i+1}\langle v_{i+1},u\rangle|\le 2, 
\end{equation} and \begin{equation}
    \mathop{\E}\limits_{\omega_{i+1}}[e^{\langle\omega_{i+1},u\rangle^{2}}] \le e^{4}.
\end{equation} If $x_{i+1}\ge \|v_{i+1}\|_{2}$ ,($x_{i+1}\le -\|v_{i+1}\|_{2}$ is the same): \begin{align}
     (\ref{eq_hy_in_subgaussian}) &= \mathop{\E}\limits_{\omega_{i}} [e^{\langle\omega_{i},u\rangle^{2}+\langle v_{i+1},u\rangle^{2}}\cdot \left(q(x_{i+1},\|v_{i+1}\|_{2})\cdot e^{2x_{i+1}\|v_{i+1}\|_{2}}+(1-q(x_{i+1},\|v_{i+1}\|_{2}))\cdot e^{-2x_{i+1}\|v_{i+1}\|_{2}}\right)]\\
     &\le \mathop{\E}\limits_{\omega_{i}} [e^{\langle\omega_{i},u\rangle^{2}+\langle v_{i+1},u\rangle^{2}}\cdot (q(x_{i+1},\|v_{i+1}\|_{2})\cdot e^{2x_{i+1}\|v_{i+1}\|_{2}}+e^{-2x_{i+1}\|v_{i+1}\|_{2}})]\\
     &\le \mathop{\E}\limits_{\omega_{i}}[exp(\langle\omega_{i},u\rangle^{2}+\langle v_{i+1},u\rangle^{2}-x_{i+1}\|v_{i+1}\|_{2})]\\
     &\le \mathop{\E}\limits_{\omega_{i}}[exp(\langle\omega_{i},u\rangle^{2}+\langle v_{i+1},u\rangle^{2}-\|v_{i+1}\|_{2}^{2})]\\
     &\le \mathop{\E}\limits_{\omega_{i}}[e^{\langle\omega_{i},u\rangle^{2}}]\\
     &\le e^{4}.
\end{align}

In a word, we have proven that for any direction $u\in \R^{n}$, by the random walk above $\langle \omega_{n}, u\rangle$ is a sub-gaussian for any $n\in \mathbb{N}$ with $\mathop{\E}\limits_{\omega_{n}}[e^{\langle\omega_{n},u\rangle^{2}}]\le e^{4}$. It implies that \begin{equation}
    \mathop{\Pr}\limits_{\omega_{n}}[|\langle \omega_{n}, u\rangle|\ge C]\le \mathop{\E}\limits_{\omega_{n}}[e^{\langle\omega_{n},u\rangle^{2}}]/C^{2} <1.
\end{equation} for any constant $C>e^{2}$. It means for any $\{v_{k}\}_{k=1}^{m}\subset \R^{n}$ with $\|v_{k}\|_{2}^{2}\le 1$, $\forall k\in [m]$, there exists an assignment $x\in \left\{ \pm 1 \right\}^{m}$ such that \begin{equation}
    \|\sum_{i=1}^{m}x_{i}\cdot v_{i}\|_{\infty}\le C.
\end{equation}
\textcolor{red}{Haoyu: Why must the transition probability $q(x,y)$ rely on the choosen direction $u$? Because if it only depends on $\langle\omega_{i},v_{i+1}\rangle$, consider the orthogonal case, in which we choose $\epsilon_{i+1} = \{\pm 1\}$ with the same probability $0.5$. Thus we need to prove\begin{equation}
  e^{\langle v_{i+1},u\rangle^{2}}\cdot \mathop{\E}\limits_{\omega_{i}}[0.5\cdot e^{\langle\omega_{i},u\rangle^{2}+\langle\omega_{i},u\rangle\cdot \langle v_{i+1},u\rangle}+0.5\cdot e^{\langle\omega_{i},u\rangle^{2}-\langle\omega_{i},u\rangle\cdot \langle v_{i+1},u\rangle}] \le C
\end{equation}
with the only assumptions \begin{equation}
    \mathop{\E}\limits_{\omega_{i}}[e^{\langle\omega_{i},u\rangle^{2}}]\le C
\end{equation}
and \begin{equation}
    \langle\omega_{i},v_{i+1}\rangle \approx 0,
\end{equation} which seems too hard to prove without the distribution of $\omega_{i}$.
} 

